Improved Multi-Scale Grid Rendering of Point Clouds for Radar Object Detection Networks

Architectures that first convert point clouds to a grid representation and then apply convolutional neural networks achieve good performance for radar-based object detection. However, the transfer from irregular point cloud data to a dense grid structure is often associated with a loss of information, due to the discretization and aggregation of points. In this paper, we propose a novel architecture, multi-scale KPPillarsBEV, that aims to mitigate the negative effects of grid rendering. Specifically, we propose a novel grid rendering method, KPBEV, which leverages the descriptive power of kernel point convolutions to improve the encoding of local point cloud contexts during grid rendering. In addition, we propose a general multi-scale grid rendering formulation to incorporate multi-scale feature maps into convolutional backbones of detection networks with arbitrary grid rendering methods. We perform extensive experiments on the nuScenes dataset and evaluate the methods in terms of detection performance and computational complexity. The proposed multi-scale KPPillarsBEV architecture outperforms the baseline by 5.37% and the previous state of the art by 2.88% in Car AP4.0 (average precision for a matching threshold of 4 meters) on the nuScenes validation set. Moreover, the proposed single-scale KPBEV grid rendering improves the Car AP4.0 by 2.90% over the baseline while maintaining the same inference speed.

==> graphics/01_teaser/structure.tex <==
\begin{tikzpicture}[node distance=1.5cm]

\def\xslant{-1}
\def\yslant{.5}
\def\gridscale{0.45}
\def\pointwidth{3pt}
\def\textdistance{0.85}
\def\labeloffset{0.75}
\definecolor{point_color}{RGB}{252,98,3}%{0,255,132}
\definecolor{invalid_point_color}{RGB}{235,235,235}
\definecolor{anchor_color}{RGB}{0,0,0}
\definecolor{empty_cell_color}{RGB}{235,235,235}
\definecolor{conv_color}{RGB}{252, 207, 3}

\tikzstyle{shadow}=[blur shadow={shadow blur steps=5,shadow blur extra rounding=1.3pt}]
\tikzstyle{annotation}=[align=center]
\tikzstyle{backbone}=[rectangle, draw, thick, minimum width=0.8cm, minimum height=1.8cm, yslant=0.5, fill=white]
\tikzstyle{default_point_style}=[point_color]
\tikzstyle{invalid_point_style}=[invalid_point_color,draw=black]
\tikzstyle{stage}=[minimum height=3.7cm, inner sep=0.2cm]


\pgfdeclarelayer{background}
\pgfsetlayers{background,main}

% Definition of input points
\newcommand{\points}[2] {
	% cell(0,1)
	\fill[#1] (0.8, 1.25) circle (\pointwidth);
	% cell(1,2)
	\fill[#1] (1.3, 2.4) circle (\pointwidth);
	% cell(1,1)
	\fill[#1] (1.3, 1.7) circle (\pointwidth);
	\fill[#1] (1.8, 1.2) circle (\pointwidth);

	% points outside the convolution radius
	% cell(0,1)
	\fill[#2] (0.35, 1.8) circle (\pointwidth);
	% cell(1,0)
	\fill[#1] (1.2, 0.8) circle (\pointwidth);
	\fill[#2] (1.6, 0.3) circle (\pointwidth);
	% cell(2,1)
	\fill[#1] (2.3, 1.8) circle (\pointwidth);
	% cell(2,2)
	\fill[#2] (2.2, 2.6) circle (\pointwidth);
	%\fill[#2] (2.8, 2.9) circle (\pointwidth);
}

\newcommand{\stageborder}[2]{
	\begin{pgfonlayer}{background}
	\draw [thick] ($(#1.north east)-(#2,0)$) -- ($(#1.north west)-(#2,0)$);
	\draw [thick] ($(#1.north west)-(#2,0)$) -- (#1.west);
	\draw [thick] ($(#1.south west)-(#2,0)$) -- (#1.west);
	%\draw [thick] (#1.north west) -- (#1.south west);
	\draw [thick] ($(#1.south west)-(#2,0)$) -- ($(#1.south east)-(#2,0)$);
	\draw [thick] ($(#1.north east)-(#2,0)$) -- (#1.east);
	\draw [thick] ($(#1.south east)-(#2,0)$) -- (#1.east);
	\end{pgfonlayer}
}

\newcommand{\stagelabel}[2]{
	\begin{pgfonlayer}{background}
	\node [inner sep=0.05cm,align=center,font=\Large] at (#2) {#1};
	\end{pgfonlayer}
}

\newcommand{\kpconv} [1]{
	\fill[conv_color, opacity=0.2] (#1) circle (1.);
	\draw[dashed, thick] (#1) circle (1.);
}


%% pointcloud
\node (pointcloud) {
	\begin{tikzpicture}
	%% nodes
	\fill[point_color] (.5,.6) circle (2.5pt);
	\fill[point_color] (0,0) circle (2.5pt);
	\fill[point_color] (-.2,.7) circle (2.5pt);
	\fill[point_color] (-.5,-.4) circle (2.5pt);
	\fill[point_color] (0,-.5) circle (2.5pt);
	\fill[point_color] (.5,-.6) circle (2.5pt);
	\end{tikzpicture}	
};


% KPBEV
\node[stage] (rendering) at ($(pointcloud)+(3.6cm,0)$) {
	\begin{tikzpicture}
	\begin{scope}[scale=0.65, yslant=\yslant,xslant=\xslant]
	\draw[thick,black,fill=white,shadow] (0,0) rectangle (3,3);
	\draw[step=1.,black] (0,0) grid (3,3);
	\kpconv{1.5,1.5}
	\points{default_point_style}{invalid_point_style}
	\fill[black] (1.5, 1.5) circle (\pointwidth);
	
	\end{scope}

	\end{tikzpicture}
};
\node[align=center,inner sep=0.03cm,fill=white, font=\large] (kplabel) at ($(rendering)+(-1.2cm,1.3cm)$) {kernel point\\convolution};
\draw ($(kplabel.south)$) -- ($(rendering)+(-0.7cm,0.35cm)$);
%\node[below=0.5cm of rendering.north] {KPBEV};
\stageborder{rendering}{0.5cm}
\node (labelheight) at ($(rendering.south)-(0,0)$) {};
\node [align=center, font=\Large] at (pointcloud.south|-labelheight.south) {point\\cloud};
\stagelabel{KPBEV\\grid rendering}{$(rendering.south)-(0.3cm,\labeloffset)$}
%\node [fill=white, inner sep=0.05cm] at ($(rendering.south)+(-0.3cm,0)$) {KPBEV};


% Grid rendering
\node[stage, minimum width=3.7cm] (gridrendering) at ($(rendering)+(4.15cm,0cm)$) {
	\begin{tikzpicture}
	% Grid 1
	\begin{scope}[yslant=\yslant,xslant=\xslant, scale=\gridscale]
		\fill[thick, draw=black, fill=white, shadow] (0,0) rectangle (3,3);
		
		\fill[point_color, rounded corners=0, opacity=0.6] (3/4,0) rectangle (6/4,3/4);
		\fill[point_color, rounded corners=0, opacity=1] (0,3/4) rectangle (3/4,6/4);
		\fill[point_color, rounded corners=0, opacity=0.3] (6/4,0) rectangle (9/4,3/4);
		\fill[point_color, rounded corners=0, opacity=0.3] (0,6/4) rectangle (3/4,9/4);
		\draw[step=3/4,black] (0,0) grid (3,3);
		\draw (3.8,0) circle (0);
	\end{scope}
	% Grid 2
	\begin{scope}[shift={(0,.3)}, yslant=\yslant,xslant=\xslant, scale=\gridscale]
		\fill[thick, draw=black, fill=white, shadow] (0,0) rectangle (3,3);
		
		\fill[point_color, rounded corners=0, opacity=0.6] (1,0) rectangle (2,1);
		\fill[point_color, rounded corners=0, opacity=1] (1,1) rectangle (2,2);
		\fill[point_color, rounded corners=0, opacity=0.4] (1,2) rectangle (2,3);
		\fill[point_color, rounded corners=0, opacity=0.8] (0,1) rectangle (1,2);
		\fill[point_color, rounded corners=0, opacity=0.5] (2,1) rectangle (3,2);
		\fill[point_color, rounded corners=0, opacity=0.3] (2,2) rectangle (3,3);
		\draw[step=1.,black] (0,0) grid (3,3);
	\end{scope}
	\begin{scope}[scale=\gridscale]
		\fill[fill=black](0, 2.3) circle (5pt);
		\fill[fill=black](0, 2.9) circle (5pt);
		\fill[fill=black](0, 3.5) circle (5pt);
	\end{scope}
	% Grid 3
	\begin{scope}[shift={(0,1.6)}, yslant=\yslant,xslant=\xslant, scale=\gridscale]
		\fill[thick, draw=black, fill=white, shadow] (0,0) rectangle (3,3);
		\fill[point_color, rounded corners=0, opacity=1] (0,0) rectangle (1.5,1.5);
		\fill[point_color, rounded corners=0, opacity=0.5] (1.5,1.5) rectangle (3,3);
		\draw[step=1.5,black] (0,0) grid (3,3);
	\end{scope}
	\end{tikzpicture}
};
\stageborder{gridrendering}{0.5cm}
\stagelabel{multi-scale\\feature maps}{$(gridrendering.south)-(0.3cm,\labeloffset)$}

% backbone
\node[stage, align=center, minimum width=3.5cm] at ($(gridrendering)+(3.75cm,0cm)$) (backbone) {
\begin{tikzpicture}
	\node [backbone] at (0,0) {};
	\node [backbone] at (0.5,0) {};
	\node [backbone] at (1.,0) {};
	\node [backbone] at (1.5,0) {};
\end{tikzpicture}
};
\stageborder{backbone}{0.5cm}
\stagelabel{CNN-based\\detector}{$(backbone.south)-(0.3cm,\labeloffset)$}

\node (bbox) at ($(backbone)+(2.7cm,0cm)$) {
	\begin{tikzpicture}
	%% nodes
	\node [thick, rectangle, minimum width=0.8cm, minimum height=0.4cm, draw=point_color, dashed, rotate=30] at (0, 0.4cm) (bb1) {};
%	\node [text=point_color] at ($(bb1)+(-0.25,0.35)$) {car};
	\node [thick, rectangle, minimum width=0.82cm, minimum height=0.45cm, draw=point_color, dashed, rotate=-5] at (0.1, -0.5cm) (bb2) {};
%	\node [text=point_color] at ($(bb2)+(0,-0.45)$) {bus};
	\end{tikzpicture}	
};
\node [align=center, font=\Large] at (bbox.south|-labelheight.south) {bounding\\boxes};

\end{tikzpicture}

==> graphics/03_kpbev/left_side.tex <==
\def\nodedistance{1cm}
%\begin{tikzpicture}[node distance=\nodedistance]

\definecolor{boxcolor}{RGB}{252,98,3}

\def\boxwidth{2.2cm}
\def\boxheight{0.6cm}
\tikzstyle{common}=[minimum width=\boxwidth, minimum height=\boxheight, rounded corners=0.1cm, ]%font=\bfseries]
\tikzstyle{kpconv}=[fill=boxcolor, text=white, common]
\tikzstyle{linear}=[draw=boxcolor,thick,common]
\tikzstyle{proj}=[fill=boxcolor, text=white, common]
\tikzstyle{dimension}=[midway,right]

\node[linear] (l0) {Linear};
\draw[-stealth] ($(l0.north)+(0,0.75)$) -- node[dimension] {$[N_\textnormal{in}, F_\textnormal{in}+7]$} (l0);

\node[kpconv, below of=l0] (l1) {KPConv};
\draw[-stealth] (l0) -- node[dimension, fill=white] {$[N_\textnormal{in}, F_\textnormal{out}]$} (l1);
\node[linear, below of=l1] (l2) {Linear};
\draw[-stealth] (l1) -- node[dimension, fill=white] (test) {$[N_\textnormal{a}, F_\textnormal{out}]$} (l2);

\node[proj, below of=l2] (l3) {Grid-Transfer};
\draw[-stealth] (l2) -- node[dimension] {$[N_\textnormal{a}, F_\textnormal{out}]$} (l3);
\draw[-stealth] (l3) -- node[dimension] {$[W, H, F_\textnormal{out}]$}  ($(l3.south)-(0,0.75)$);



%\end{tikzpicture}


==> graphics/03_kpbev/right_side.tex <==
\begin{tikzpicture}

\def\xslant{-1}
\def\yslant{.5}
\def\gridscale{0.55}
\def\pointwidth{2pt}
\def\textdistance{0.85}
\definecolor{point_color}{RGB}{252,98,3}%{0,255,132}
\definecolor{invalid_point_color}{RGB}{235,235,235}
\definecolor{anchor_color}{RGB}{0,0,0}
\definecolor{empty_cell_color}{RGB}{235,235,235}
\definecolor{conv_color}{RGB}{252, 207, 3}

\tikzstyle{annotation}=[align=center]
\tikzstyle{default_point_style}=[point_color]
\tikzstyle{invalid_point_style}=[invalid_point_color,draw=black]

% Definition of input points
\newcommand{\points}[2] {
	% cell(0,1)
	\fill[#1] (0.7, 1.2) circle (\pointwidth);
	% cell(1,0)
	\fill[#1] (1.2, 0.8) circle (\pointwidth);
	\fill[#1] (1.6, 0.6) circle (\pointwidth);
	% cell(1,1)
	\fill[#1] (1.2, 1.7) circle (\pointwidth);
	\fill[#1] (1.7, 1.3) circle (\pointwidth);
	\fill[#1] (1.8, 1.9) circle (\pointwidth);
	% cell(1,2)
	\fill[#1] (2.3, 1.8) circle (\pointwidth);
	
	% points outside the convolution radius
	% cell(0,1)
	\fill[#2] (0.4, 1.8) circle (\pointwidth);
	% cell(1,0)
	\fill[#2] (1.5, 0.2) circle (\pointwidth);
	% cell(2,2)
	\fill[#2] (2.4, 2.2) circle (\pointwidth);
	\fill[#2] (2.2, 2.4) circle (\pointwidth);
	\fill[#2] (2.8, 2.9) circle (\pointwidth);
	
}

% Definition of anchor points
\newcommand{\anchors} {
	% cell(0,1)
	\fill[anchor_color] (0.5, 1.5) circle (\pointwidth);
	% cell(1,0)
	\fill[anchor_color] (1.5, 0.5) circle (\pointwidth);
	% cell(1,1)
	\fill[anchor_color] (1.5, 1.5) circle (\pointwidth);
	% cell(1,2)
	\fill[anchor_color] (2.5, 1.5) circle (\pointwidth);
	%cell(2,2)
	\fill[anchor_color] (2.5, 2.5) circle (\pointwidth);
}

% Definition of grid
\newcommand{\grid} {
	% empty cells
	\fill[empty_cell_color, rounded corners=0] (0,0) rectangle (1,1);
	\fill[empty_cell_color, rounded corners=0] (2,0) rectangle (3,1);
	\fill[empty_cell_color, rounded corners=0] (0,2) rectangle (1,3);
	\fill[empty_cell_color, rounded corners=0] (1,2) rectangle (2,3);
	
	\draw[step=1.,black,] (-0.25,-0.25) grid (3.25, 3.25);
}

% Definition of convolution radius
\newcommand{\kpconv} {

	% convolution radius
	\fill[conv_color, opacity=0.2] (1.5, 1.5) circle (1);
	\draw[dashed, thick] (1.5, 1.5) circle (1);
		
	\draw[stealth-stealth] ($(1.5, 1.5)+(0,\pointwidth)$) -- node [midway,above,xshift=1pt,yshift=-1pt] {\large$\rho$} (1.5, 2.5);
	\node (neighborhood) at (4., 2.3) {\large$\mathcal{N}_\textnormal{a}$};
	\draw ($(neighborhood.south west)+(0.2,0.1)$) -- (2.2, 1.4);
}

% Grid projection
\node[scale=\gridscale] (projection) {
\begin{tikzpicture}
	\begin{scope}[yslant=\yslant,xslant=\xslant]
	\points{default_point_style}{default_point_style}
	\grid
	\draw [stealth-stealth] (1,-0.45) -- node[midway, below] {\large $s$}  (2,-0.45);
	\end{scope}
	%\draw [stealth-stealth] ($(projection.east)+(-1.1,-0.65)$) -- node[midway, below] {\large $r$} ($(projection.east)+(-0.55,-0.39)$);
\end{tikzpicture}

};
\begin{scope}[scale=\gridscale]

\end{scope}

\node[annotation] at ($(projection.east)+(\textdistance,0)$) {grid\\projection};

% Anchor generation
\node[anchor=north, scale=\gridscale] (anchors) at (projection.south) {
\begin{tikzpicture}
	\begin{scope}[yslant=\yslant,xslant=\xslant]
		\anchors
		\grid
	\end{scope}
\end{tikzpicture}
};
\node[annotation] at ($(anchors.east)+(\textdistance,0)$) {anchor\\generation};

% Kernel point convolution
\node[anchor=north, scale=\gridscale] (kpconv) at (anchors.south) {
\begin{tikzpicture}
	\begin{scope}[yslant=\yslant,xslant=\xslant]
		\grid
		\kpconv
		\points{default_point_style}{invalid_point_style}
		\fill[anchor_color] (1.5, 1.5) circle (\pointwidth);
	\end{scope}
\end{tikzpicture}
};
\node[annotation] at ($(kpconv.east)+(\textdistance,0)$) {kernel point\\conv. \eq{eq:kpconv}};
\end{tikzpicture}

==> graphics/04_complexity/na_to_nin.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate213940}{RGB}{213,94,0}
\definecolor{darkcyan1115178}{RGB}{1,115,178}
\definecolor{darkcyan2158115}{RGB}{2,158,115}
\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{darkorange2221435}{RGB}{222,143,5}
\definecolor{orchid204120188}{RGB}{204,120,188}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={\(\displaystyle N_{a}/N_{in}\)},
xmajorgrids,
xmin=0.178294573643411, xmax=1,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Number of occurences},
ymajorgrids,
ymin=0, ymax=443.1,
ytick style={color=black}
]
\addplot [thick, darkcyan1115178]
table {%
	0.178294573643411 4
	0.183777797731286 3
	0.189261021819161 8
	0.194744245907037 16
	0.200227469994912 15
	0.205710694082787 23
	0.211193918170662 17
	0.216677142258538 28
	0.222160366346413 28
	0.227643590434288 34
	0.233126814522163 38
	0.238610038610039 37
	0.244093262697914 35
	0.249576486785789 34
	0.255059710873664 47
	0.26054293496154 59
	0.266026159049415 56
	0.27150938313729 72
	0.276992607225165 80
	0.282475831313041 128
	0.287959055400916 136
	0.293442279488791 189
	0.298925503576666 193
	0.304408727664542 249
	0.309891951752417 311
	0.315375175840292 322
	0.320858399928167 344
	0.326341624016043 361
	0.331824848103918 350
	0.337308072191793 347
	0.342791296279668 333
	0.348274520367544 327
	0.353757744455419 308
	0.359240968543294 248
	0.364724192631169 219
	0.370207416719045 171
	0.37569064080692 129
	0.381173864894795 118
	0.38665708898267 109
	0.392140313070546 60
	0.397623537158421 55
	0.403106761246296 44
	0.408589985334171 44
	0.414073209422047 34
	0.419556433509922 31
	0.425039657597797 16
	0.430522881685672 11
	0.436006105773548 11
	0.441489329861423 7
	0.446972553949298 11
	0.452455778037173 3
	0.457939002125049 3
	0.463422226212924 4
	0.468905450300799 1
	0.474388674388674 1
	0.47987189847655 1
	0.485355122564425 2
	0.4908383466523 1
	0.496321570740175 1
	0.501804794828051 0
	0.507288018915926 1
	0.512771243003801 0
	0.518254467091676 0
	0.523737691179552 1
	0.529220915267427 0
	0.534704139355302 0
	0.540187363443177 0
	0.545670587531053 0
	0.551153811618928 0
	0.556637035706803 0
	0.562120259794678 0
	0.567603483882554 0
	0.573086707970429 0
	0.578569932058304 0
	0.584053156146179 0
	0.589536380234055 0
	0.59501960432193 0
	0.600502828409805 0
	0.60598605249768 0
	0.611469276585556 0
	0.616952500673431 0
	0.622435724761306 0
	0.627918948849181 0
	0.633402172937057 0
	0.638885397024932 0
	0.644368621112807 0
	0.649851845200683 0
	0.655335069288558 0
	0.660818293376433 0
	0.666301517464308 0
	0.671784741552183 0
	0.677267965640059 0
	0.682751189727934 0
	0.688234413815809 0
	0.693717637903684 0
	0.69920086199156 0
	0.704684086079435 1
	0.71016731016731 1
	0.715650534255185 2
	0.721133758343061 0
	0.726616982430936 0
	0.732100206518811 0
	0.737583430606687 4
	0.743066654694562 1
	0.748549878782437 4
	0.754033102870312 0
	0.759516326958187 2
	0.764999551046063 2
	0.770482775133938 4
	0.775965999221813 6
	0.781449223309688 4
	0.786932447397564 4
	0.792415671485439 5
	0.797898895573314 7
	0.80338211966119 5
	0.808865343749065 5
	0.81434856783694 9
	0.819831791924815 10
	0.825315016012691 5
	0.830798240100566 10
	0.836281464188441 10
	0.841764688276316 6
	0.847247912364192 3
	0.852731136452067 4
	0.858214360539942 3
	0.863697584627817 5
	0.869180808715692 3
	0.874664032803568 5
	0.880147256891443 3
	0.885630480979318 5
	0.891113705067194 2
	0.896596929155069 1
	0.902080153242944 1
	0.907563377330819 1
	0.913046601418695 1
	0.91852982550657 1
	0.924013049594445 2
	0.92949627368232 0
	0.934979497770196 0
	0.940462721858071 1
};
\addplot [thick, darkorange2221435]
table {%
	0.207430340557276 3
	0.213338465400385 2
	0.219246590243494 10
	0.225154715086604 17
	0.231062839929713 23
	0.236970964772822 31
	0.242879089615932 44
	0.248787214459041 36
	0.25469533930215 34
	0.26060346414526 26
	0.266511588988369 39
	0.272419713831479 42
	0.278327838674588 50
	0.284235963517697 44
	0.290144088360807 36
	0.296052213203916 55
	0.301960338047025 53
	0.307868462890135 71
	0.313776587733244 85
	0.319684712576353 89
	0.325592837419463 102
	0.331500962262572 126
	0.337409087105682 174
	0.343317211948791 219
	0.3492253367919 251
	0.35513346163501 332
	0.361041586478119 300
	0.366949711321228 319
	0.372857836164338 404
	0.378765961007447 371
	0.384674085850557 328
	0.390582210693666 353
	0.396490335536775 308
	0.402398460379885 265
	0.408306585222994 249
	0.414214710066103 209
	0.420122834909213 164
	0.426030959752322 128
	0.431939084595431 103
	0.437847209438541 86
	0.44375533428165 62
	0.449663459124759 52
	0.455571583967869 40
	0.461479708810978 38
	0.467387833654088 23
	0.473295958497197 22
	0.479204083340306 8
	0.485112208183416 13
	0.491020333026525 7
	0.496928457869634 4
	0.502836582712744 5
	0.508744707555853 2
	0.514652832398963 1
	0.520560957242072 2
	0.526469082085181 2
	0.532377206928291 1
	0.5382853317714 0
	0.544193456614509 2
	0.550101581457619 3
	0.556009706300728 0
	0.561917831143837 1
	0.567825955986947 0
	0.573734080830056 0
	0.579642205673165 0
	0.585550330516275 0
	0.591458455359384 0
	0.597366580202494 0
	0.603274705045603 0
	0.609182829888712 0
	0.615090954731822 0
	0.620999079574931 0
	0.62690720441804 0
	0.63281532926115 0
	0.638723454104259 0
	0.644631578947368 0
	0.650539703790478 0
	0.656447828633587 0
	0.662355953476697 0
	0.668264078319806 0
	0.674172203162915 0
	0.680080328006025 0
	0.685988452849134 0
	0.691896577692243 0
	0.697804702535353 0
	0.703712827378462 0
	0.709620952221572 0
	0.715529077064681 0
	0.72143720190779 0
	0.7273453267509 0
	0.733253451594009 0
	0.739161576437118 0
	0.745069701280228 0
	0.750977826123337 0
	0.756885950966447 1
	0.762794075809556 1
	0.768702200652665 0
	0.774610325495775 1
	0.780518450338884 1
	0.786426575181993 1
	0.792334700025103 1
	0.798242824868212 3
	0.804150949711321 5
	0.810059074554431 2
	0.81596719939754 7
	0.821875324240649 5
	0.827783449083759 11
	0.833691573926868 9
	0.839599698769977 12
	0.845507823613087 6
	0.851415948456196 9
	0.857324073299306 2
	0.863232198142415 14
	0.869140322985524 8
	0.875048447828634 7
	0.880956572671743 6
	0.886864697514852 6
	0.892772822357962 7
	0.898680947201071 4
	0.90458907204418 3
	0.91049719688729 4
	0.916405321730399 6
	0.922313446573509 1
	0.928221571416618 2
	0.934129696259727 0
	0.940037821102837 3
};
\addplot [thick, darkcyan2158115]
table {%
	0.244582043343653 4
	0.251604899902114 4
	0.258627756460574 8
	0.265650613019034 19
	0.272673469577494 28
	0.279696326135955 30
	0.286719182694415 24
	0.293742039252875 34
	0.300764895811335 27
	0.307787752369796 31
	0.314810608928256 32
	0.321833465486716 33
	0.328856322045177 36
	0.335879178603637 42
	0.342902035162097 35
	0.349924891720557 35
	0.356947748279018 30
	0.363970604837478 30
	0.370993461395938 27
	0.378016317954398 38
	0.385039174512859 26
	0.392062031071319 40
	0.399084887629779 38
	0.40610774418824 25
	0.4131306007467 41
	0.42015345730516 25
	0.42717631386362 36
	0.434199170422081 38
	0.441222026980541 55
	0.448244883539001 66
	0.455267740097461 96
	0.462290596655922 130
	0.469313453214382 146
	0.476336309772842 168
	0.483359166331303 231
	0.490382022889763 262
	0.497404879448223 298
	0.504427736006683 363
	0.511450592565144 400
	0.518473449123604 404
	0.525496305682064 352
	0.532519162240525 369
	0.539542018798985 316
	0.546564875357445 308
	0.553587731915905 256
	0.560610588474366 189
	0.567633445032826 173
	0.574656301591286 115
	0.581679158149746 93
	0.588702014708207 71
	0.595724871266667 46
	0.602747727825127 38
	0.609770584383587 28
	0.616793440942048 24
	0.623816297500508 13
	0.630839154058968 13
	0.637862010617429 10
	0.644884867175889 7
	0.651907723734349 3
	0.658930580292809 2
	0.66595343685127 1
	0.67297629340973 0
	0.67999914996819 5
	0.68702200652665 1
	0.694044863085111 0
	0.701067719643571 0
	0.708090576202031 1
	0.715113432760492 0
	0.722136289318952 0
	0.729159145877412 0
	0.736182002435872 0
	0.743204858994333 0
	0.750227715552793 0
	0.757250572111253 0
	0.764273428669713 0
	0.771296285228174 0
	0.778319141786634 0
	0.785341998345094 0
	0.792364854903555 0
	0.799387711462015 0
	0.806410568020475 0
	0.813433424578935 0
	0.820456281137396 0
	0.827479137695856 0
	0.834501994254316 0
	0.841524850812777 0
	0.848547707371237 1
	0.855570563929697 0
	0.862593420488157 3
	0.869616277046618 1
	0.876639133605078 7
	0.883661990163538 6
	0.890684846721998 11
	0.897707703280459 4
	0.904730559838919 14
	0.911753416397379 15
	0.91877627295584 16
	0.9257991295143 16
	0.93282198607276 20
	0.93984484263122 11
	0.946867699189681 7
	0.953890555748141 9
	0.960913412306601 4
	0.967936268865061 2
	0.974959125423522 1
};
\addplot [thick, chocolate213940]
table {%
	0.269372693726937 1
	0.276519008071006 1
	0.283665322415075 6
	0.290811636759143 9
	0.297957951103212 21
	0.305104265447281 19
	0.31225057979135 25
	0.319396894135418 25
	0.326543208479487 21
	0.333689522823556 24
	0.340835837167624 21
	0.347982151511693 19
	0.355128465855762 25
	0.36227478019983 33
	0.369421094543899 32
	0.376567408887968 36
	0.383713723232036 31
	0.390860037576105 32
	0.398006351920174 26
	0.405152666264243 28
	0.412298980608311 23
	0.41944529495238 32
	0.426591609296449 31
	0.433737923640517 22
	0.440884237984586 25
	0.448030552328655 37
	0.455176866672724 30
	0.462323181016792 23
	0.469469495360861 27
	0.47661580970493 22
	0.483762124048998 16
	0.490908438393067 14
	0.498054752737136 13
	0.505201067081204 12
	0.512347381425273 17
	0.519493695769342 13
	0.526640010113411 17
	0.533786324457479 22
	0.540932638801548 23
	0.548078953145616 34
	0.555225267489685 38
	0.562371581833754 56
	0.569517896177823 86
	0.576664210521891 105
	0.58381052486596 149
	0.590956839210029 180
	0.598103153554097 215
	0.605249467898166 244
	0.612395782242235 295
	0.619542096586304 334
	0.626688410930372 383
	0.633834725274441 377
	0.64098103961851 415
	0.648127353962578 377
	0.655273668306647 361
	0.662419982650716 299
	0.669566296994784 259
	0.676712611338853 192
	0.683858925682922 173
	0.691005240026991 113
	0.698151554371059 107
	0.705297868715128 64
	0.712444183059197 42
	0.719590497403265 33
	0.726736811747334 24
	0.733883126091403 19
	0.741029440435471 12
	0.74817575477954 12
	0.755322069123609 2
	0.762468383467678 7
	0.769614697811746 2
	0.776761012155815 3
	0.783907326499884 2
	0.791053640843952 1
	0.798199955188021 0
	0.80534626953209 0
	0.812492583876158 0
	0.819638898220227 0
	0.826785212564296 0
	0.833931526908365 0
	0.841077841252433 0
	0.848224155596502 0
	0.855370469940571 0
	0.862516784284639 0
	0.869663098628708 0
	0.876809412972777 0
	0.883955727316845 0
	0.891102041660914 1
	0.898248356004983 0
	0.905394670349052 1
	0.91254098469312 3
	0.919687299037189 6
	0.926833613381258 5
	0.933979927725326 12
	0.941126242069395 15
	0.948272556413464 15
	0.955418870757533 21
	0.962565185101601 30
	0.96971149944567 24
	0.976857813789739 13
	0.984004128133807 2
};
\addplot [thick, orchid204120188]
table {%
	0.333745364647713 1
	0.339488939090405 1
	0.345232513533097 2
	0.35097608797579 1
	0.356719662418482 2
	0.362463236861174 4
	0.368206811303866 10
	0.373950385746558 9
	0.37969396018925 10
	0.385437534631942 15
	0.391181109074634 18
	0.396924683517327 17
	0.402668257960019 16
	0.408411832402711 15
	0.414155406845403 19
	0.419898981288095 11
	0.425642555730787 14
	0.431386130173479 25
	0.437129704616172 13
	0.442873279058864 23
	0.448616853501556 13
	0.454360427944248 23
	0.46010400238694 22
	0.465847576829632 26
	0.471591151272324 27
	0.477334725715016 23
	0.483078300157709 19
	0.488821874600401 21
	0.494565449043093 12
	0.500309023485785 15
	0.506052597928477 16
	0.511796172371169 20
	0.517539746813861 18
	0.523283321256553 24
	0.529026895699246 17
	0.534770470141938 27
	0.54051404458463 23
	0.546257619027322 23
	0.552001193470014 18
	0.557744767912706 22
	0.563488342355398 14
	0.56923191679809 11
	0.574975491240783 14
	0.580719065683475 7
	0.586462640126167 20
	0.592206214568859 7
	0.597949789011551 11
	0.603693363454243 4
	0.609436937896935 17
	0.615180512339627 6
	0.62092408678232 5
	0.626667661225012 8
	0.632411235667704 10
	0.638154810110396 8
	0.643898384553088 9
	0.64964195899578 10
	0.655385533438472 7
	0.661129107881165 12
	0.666872682323857 11
	0.672616256766549 13
	0.678359831209241 9
	0.684103405651933 6
	0.689846980094625 10
	0.695590554537317 4
	0.701334128980009 12
	0.707077703422701 11
	0.712821277865394 9
	0.718564852308086 13
	0.724308426750778 18
	0.73005200119347 19
	0.735795575636162 22
	0.741539150078854 23
	0.747282724521546 43
	0.753026298964238 44
	0.758769873406931 79
	0.764513447849623 96
	0.770257022292315 110
	0.776000596735007 178
	0.781744171177699 204
	0.787487745620391 246
	0.793231320063083 279
	0.798974894505776 340
	0.804718468948468 359
	0.81046204339116 402
	0.816205617833852 422
	0.821949192276544 389
	0.827692766719236 386
	0.833436341161928 321
	0.83917991560462 274
	0.844923490047312 217
	0.850667064490005 152
	0.856410638932697 118
	0.862154213375389 74
	0.867897787818081 54
	0.873641362260773 30
	0.879384936703465 18
	0.885128511146157 19
	0.89087208558885 12
	0.896615660031542 2
	0.902359234474234 5
	0.908102808916926 0
	0.913846383359618 1
	0.91958995780231 0
	0.925333532245002 0
	0.931077106687695 0
	0.936820681130387 1
	0.942564255573079 1
	0.948307830015771 0
	0.954051404458463 2
	0.959794978901155 1
	0.965538553343847 8
	0.971282127786539 13
	0.977025702229231 25
	0.982769276671924 31
	0.988512851114616 40
	0.994256425557308 26
};
\draw (axis cs:0.368,190.323668122271) node[
scale=0.8,
text=darkcyan1115178,
rotate=273.6,
fill=white,
inner sep=0.05cm
]{$s=1.5\,m$};
\draw (axis cs:0.417,187.785477566282) node[
scale=0.8,
text=darkorange2221435,
rotate=274.2,
fill=white,
inner sep=0.05cm
]{$s=1.25\,m$};
\draw (axis cs:0.56,194.825183448066) node[
scale=0.8,
text=darkcyan2158115,
rotate=273.3,
fill=white,
inner sep=0.05cm
]{$s=0.75\,m$};
\draw (axis cs:0.675,208.056522870198) node[
scale=0.8,
text=chocolate213940,
rotate=273.4,
fill=white,
inner sep=0.05cm
]{$s=0.5\,m$};
\draw (axis cs:0.845,216.13413729128) node[
scale=0.8,
text=orchid204120188,
rotate=272.8,
fill=white,
inner sep=0.05cm
]{$s=0.25\,m$};
\end{axis}

\end{tikzpicture}

==> tables/04_testset.tex <==
\begin{tabular}{l c c c c}
	\toprule
	\textbf{Object detector} &  \textbf{mAP (\%) $\uparrow$} & \textbf{ATE $\downarrow$} & \textbf{ASE $\downarrow$} & \textbf{AOE $\downarrow$}\\
	\hline
	Radar-PointGNN \cite{Svenningsson2021} & 10.1 & 0.69 & 0.20 & 0.38\\
	KPConvPillars \cite{Ulrich2022} & 29.8 & 0.589 & 0.183 & 0.336 \\
	KPPillarsBEV (ours) & \textcolor{red}{$x.x\,\%$} & \textcolor{red}{$x.x\,\%$} & \textcolor{red}{$x.x\,\%$} & \textcolor{red}{$x.x\,\%$}\\
	\bottomrule
\end{tabular}
